DAReN: A Collaborative Approach Towards Reasoning And Disentangling

Computational learning approaches to solving visual reasoning tests, such as Raven's Progressive Matrices (RPM), critically depend on the ability to identify the visual concepts used in the test (i.e., the representation) as well as the latent rules based on those concepts (i.e., the reasoning). However, learning of representation and reasoning is a challenging and ill-posed task, often approached in a stage-wise manner (first representation, then reasoning). In this work, we propose an end-to-end joint representation-reasoning learning framework, which leverages a weak form of inductive bias to improve both tasks together. Specifically, we introduce a general generative graphical model for RPMs, GM-RPM, and apply it to solve the reasoning test. We accomplish this using a novel learning framework Disentangling based Abstract Reasoning Network (DAReN) based on the principles of GM-RPM. We perform an empirical evaluation of DAReN over several benchmark datasets. DAReN shows consistent improvement over state-of-the-art (SOTA) models on both the reasoning and the disentanglement tasks. This demonstrates the strong correlation between disentangled latent representation and the ability to solve abstract visual reasoning tasks.

==> abstract.tex <==
\begin{abstract}
  % Reasoning tests, such as Raven's Progressive Matrices (RPM), have been used as a testbed over the years to evaluate human intelligence.
  % Is it possible to measure the IQ of an AI model?, Can it solve new independent problems by learning concepts?.
  % In this work, we use the true generative factors in images as a form of visual concept to evaluate the reasoning performance of a model.
  % Prior works have empirically confirmed the advantages of disentangled representation~\cite{van2019disentangled} in abstract visual reasoning.
  % However, the reasoning score remains suboptimal due to the inferior standard of representation and limitation in the network architecture which fails to exploit the hidden pattern present in the reasoning dataset.
  % %As humans who at a young age start with primitive concepts to small simpler tests and grows with experience to form complex concepts via overlaying multiple basic concepts to solve challenging tests.
  % %Similarly, an AI model needs the representation to evolve as well to solve these tests more efficiently.


  Computational learning approaches to solving visual reasoning tests, such as Raven's Progressive Matrices (RPM), critically depend on the ability of the computational approach to identify the visual concepts used in the test (i.e., the representation) as well as the latent rules based on those concepts (i.e., the reasoning).  However, learning of representation and reasoning is a challenging and ill-posed task, often approached in a stage-wise manner (first representation, then reasoning).
  In this work, we propose an end-to-end joint representation-reasoning learning framework, which leverages a weak form of inductive bias to improve both tasks together.  Specifically, we propose a general generative graphical model for RPM, \textit{GM-RPM}, and apply it to solve the reasoning test.  We accomplish this using a novel learning framework \tb{D}isentangling based \tb{A}bstract \tb{R}easoning \tb{N}etwork (\daren) based on the principles of  \textit{GM-RPM}.
  We perform an empirical evaluation of \daren over several benchmark datasets.
  \daren shows consistent improvement over state-of-the-art (SOTA) models on both the reasoning and the disentanglement tasks.
  This demonstrates the strong correlation between disentangled latent representation and the ability to solve abstract visual reasoning tasks.
  % To succeed, both the reasoning ability of the module as well as the disentangling module show work jointly to solve these tests.
  % Eventhough prior works have proposed models to solve RPM, a generalized framework has not been proposed yet.
  % In this paper, we propose a generalized framework (ref to \red{}) to solve RPM.
  % We believe that our \red{name} will provide, for the first time, a detailed understading towards solving these problems.
  % Inspired fom this, we also propose a novel model DAReN that performs joint optimization on both the disentanglement and reasoning.
  % We also extend the staged training approach in prior work ~\cite{van2019disentangled} to adapt an end--to--end training model.
\end{abstract}


==> data/graphical_model.tex <==
\begin{tikzpicture}
    % \node[latent] (rule) {$r$} ; %
    % \node[latent, above=of rule] (rel) {$o$} ; %

    \node[latent] (rule) {$r$} ; %
    \node[latent, left=of rule] (rel) {$o$} ; %

    \node[latent, below=of rule, xshift=1.5cm] (zo) {$z_o$} ; %
    % \node[latent, below=of rel, xshift=-1.0cm, yshift=0.8cm] (oc) {$o_c$} ; %
    \node[latent, below=of rel] (zoc2) {$z_{o^\complement,2}$} ; %
    \node[latent, left=of zoc2] (zoc1) {$z_{o^\complement,1}$} ; %
    \node[latent, right=of zoc2] (zoc3) {$z_{o^\complement,3}$} ; %

    \node[obs, below=of zoc3] (x2) {$x_2$} ; %
    \node[obs, left=of x2] (x1) {$x_1$} ; %
    \node[obs, right=of x2] (x3) {$x_3$} ; %
    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate1} {(zo) (zoc1) (zoc2) (zoc3) (x1) (x2) (x3)} {$M$}; %
    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate2} {(rel) (rule) (plate1)} {N}; %
    \edge {rule} {zo} ; %
    \edge {rel} {zo} ; %
    \edge {zo} {x1} ; %
    \edge {zo} {x2} ; %
    \edge {zo} {x3} ; %
    \edge {zoc1} {x1} ; %
    \edge {zoc2} {x2} ; %
    \edge {zoc3} {x3} ; %
    % \edge {rel} {oc} ; %
    \edge {rel} {zoc1} ; %
    \edge {rel} {zoc2} ; %
    \edge {rel} {zoc3} ; %
    % \edge {z,beta} {w} ; %

\end{tikzpicture}

==> data/graphical_model_1.tex <==
\begin{tikzpicture}
    % \node[latent] (rule) {$r$} ; %
    % \node[latent, above=of rule] (rel) {$o$} ; %

    \node[latent] (rule) {$r$} ; %
    % \node[latent, left=of rule] (rel) {$o$} ; %
     
    \node[latent, below=of rule] (zo) {$\mb{z}_o$} ; %
    \node[latent, right=of zo] (rel) {$\mb{o}$} ; %

    \node[latent, left=of zo] (zoc3) {$z_{o^\complement,3}$} ; %
    \node[latent, left=of zoc3] (zoc2) {$z_{o^\complement,2}$} ; %
    \node[latent, left=of zoc2] (zoc1) {$z_{o^\complement,1}$} ; %
 
    \node[latent, below=of zoc3] (z2) {$z_2$} ; %
    \node[latent, left=of z2] (z1) {$z_1$} ; %
    \node[latent, right=of z2] (z3) {$z_3$} ; %

    \node[obs, below=of z3] (x3) {$x_3$} ; %
    \node[obs, left=of x3] (x2) {$x_2$} ; %
    \node[obs, left=of x2] (x1) {$x_1$} ; %

    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate1} {(zo) (zoc1) (zoc2) (zoc3) (x1) (x2) (x3)} {$M$}; %
    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate2} {(rel) (rule) (plate1)} {N}; %

    \edge {rule} {zo} ; %
    %\edge {rel} {zo} ; %
    \edge {zo} {z1} ; %
    \edge {zo} {z2} ; %
    \edge {zo} {z3} ; %
    \edge {zoc1} {z1} ; %
    \edge {zoc2} {z2} ; %
    \edge {zoc3} {z3} ; %
    % \edge {rel} {oc} ; %
    \edge {rel} {z1} ; %
    \edge {rel} {z2} ; %
    \edge {rel} {z3} ; %
    % \edge {z,beta} {w} ; %

    \edge {z1} {x1} ; %
    \edge {z2} {x2} ; %
    \edge {z3} {x3} ; %

\end{tikzpicture}

==> data/graphical_model_2.tex <==
\begin{tikzpicture}
    % \node[latent] (rule) {$r$} ; %
    % \node[latent, above=of rule] (rel) {$o$} ; %

    % \node[latent] (okn) {$\mathcal{o}$}
    \node[latent] (rule) {$r$} ; %
    % \node[latent, left=of rule] (rel) {$o$} ; %

    \node[latent, below=of rule] (zo) {$\mb{z}_{i:,o}$} ; %
    \node[latent, left=of zo] (zoc) {$\mb{z}_{ij,\overline{o}}$} ; %

    \node[latent, right=of zo] (rel) {$\mb{o}$} ; %

    \node[latent, below=of zoc] (z) {$\mb{z}_{ij}$} ; %

    \node[latent, left=of zoc] (zn) {$\mb{z}_{ij,n}$} ; %

    \node[obs, below=of z] (x) {$\mb{x}_{ij}$} ; %

    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate0} {(zoc) (zn) (x)} {columns: $M$}; %

    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate1} {(zo) (plate0)} {rows: $M$}; %
    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate2} {(rel) (rule) (plate1)} {RPM: $D$}; %

    \edge {rule} {zo} ; %
    \edge {zo} {z} ; %
    \edge {zoc} {z} ; %
    \edge {rel} {z} ; %
    \edge {zn} {z}; %
    \edge {z} {x} ; %

\end{tikzpicture}
